PRANK: a singular value based noise filtering of multiple response datasets for experimental dynamics

High quality measurements are paramount to a successful application of experimental techniques in structural dynamics. The presence of noise and disturbances can significantly distort the information stored in the data and, if not adequately treated, may result in erroneous findings and misleading predictions. A common technique to filter out noise relies on decomposing the dataset into singular components sorted by their degree of significance. Discarding low-value contributions helps to clean the data and remove spuriousness. This paper presents PRANK, a novel singular value-based reconstruction approach for multiple response vibration datasets. PRANK integrates the effect of Principal Response Functions and Hankel filtering actions, resulting in an improved data reconstruction for both system poles and zeros. The proposed formulation is tested on both analytical and numerical examples, showcasing its robustness, efficiency and versatility. PRANK operates with both time- and frequency-based data. Applied to noisy full-field camera measurements, the filter delivered excellent performance, indicating its potential for various identification tasks and applications in vibration analysis.

==> source/sec_07.tex <==
% !TeX spellcheck = en_US
\section{Discussion}
\label{sec:Discussion}
PRANK is the idea of combining multiple flavors of TSVD based on the topological representation of the available measured MIMO spectral dataset. The filtering algorithm is incorporated within a streamlined and automated framework. The results arising from the analytical example in \cref{sec:SVR}, the numerical case in \cref{sec:NE} and the experimental application in \cref{sec:EE} display the potential of PRANK in the field of vibration analysis. PRANK focuses on the removal of random error and outliers. No systematic error is treated. Since the core of the filtering is based on a least square TSVD estimator, in a realistic scenario, namely when the conditions assumed in \cref{sec:PRANK_sec} are not fully satisfied, some distortion of the desired underlying signal will inevitably occur. For that reason, it is strongly recommended to apply PRANK on the measured data only if necessary, i.e. a 'relevant' amount of noise is visible. The interpretation of 'relevant' is up to the user and will depend on the specific application.\\
At the light of the experimental application of \cref{sec:EE}, it is worth to clarify the difference between PRANK, i.e. a SVD strategy, and a classic modal decomposition approach. Both decompose the dataset in a simple linear combination of fundamental contributions. If a modal approach seeks to find mass and stiffness orthogonal mode shapes, the singular approach retrieves orthonormal singular vectors. The information contained in the two bases is generally the same, although distributed differently. Due to its mathematical roots, PRANK is not capable of preserving physical properties of a linear time-invariant system such as passivity (see \cref{sec:PRANK_sec}) and reciprocity. Thus, if the goal is to estimate modal parameters, PRANK is not an alternative to modal identification, but rather a supplementary function (see results in \cref{fig:modes}). In this context, it could be an additional option to other existing noise removal techniques associated with modal identification (e.g. the Maximum Likelihood Modal Model estimator for Polymax \cite{El-Kafafy2013}). If, instead, the goal is to clean a dataset while preserving the dominant underlying dynamics, PRANK may be a robust alternative to a modal reconstruction/synthesis (see results in \cref{fig:Comparison_FRFs}). Further study of PRANK in combination with or as an alternative to modal identification is envisioned.\\
The potential enhancement of PRANK with physicality-preserving constraints is under research. The application of PRANK within NVH operations such as Frequency-Based Substructuring (FBS) and Transfer Path Analysis (TPA) is left for future work. 


\section{Conclusion}
\label{sec:Conclusion}
Noise and disturbances arising from experimental measurements are often unavoidable and, if not adequately treated, can lead to erroneous or incomplete findings.\\
This article presents PRANK: A robust, efficient and automated algorithm based on singular values truncation designed to remove noise and outliers from measured MIMO response datasets. The approach capitalizes on the complementary effects of PRF (to detect outliers) and of Hankel (to remove random noise) SVD truncation mechanisms. The sequential use of PRF followed by Hankel, termed as $PRANK_{PH}$, demonstrates superior effectiveness compared to employing each filtering technique independently. A novel way of mixing the two techniques, $PRANK_{HiP}$, is formulated that goes beyond a sequential application, resulting in comparable cleaning effectiveness, significantly reduced computational cost, and enhanced versatility. The selection of the truncation basis is automated through the integration of the e15 algorithm proposed in literature, which is proven applicable to NVH datasets in the form used by PRANK. An analytical example is used to show the applicability, benefits and drawbacks of different SVD truncation approaches. A numerical example shows the efficacy of the full PRANK functionality, highlighting accuracy and cost of the proposed strategy. Excellent noise removal and signal reconstruction is demonstrated in the context of a full-field camera-based experimental modal analysis. \\
Future research will be made to extend the usability and reliability of the algorithm and to investigate applications to different fields and problems.
